Paxion: Patching Action Knowledge in Video-Language Foundation Models

Action knowledge involves the understanding of textual, visual, and temporal aspects of actions. We introduce the Action Dynamics Benchmark (ActionBench) containing two carefully designed probing tasks: Action Antonym and Video Reversal, which targets multimodal alignment capabilities and temporal understanding skills of the model, respectively. Despite recent video-language models' (VidLM) impressive performance on various benchmark tasks, our diagnostic tasks reveal their surprising deficiency (near-random performance) in action knowledge, suggesting that current models rely on object recognition abilities as a shortcut for action understanding. To remedy this, we propose a novel framework, Paxion, along with a new Discriminative Video Dynamics Modeling (DVDM) objective. The Paxion framework utilizes a Knowledge Patcher network to encode new action knowledge and a Knowledge Fuser component to integrate the Patcher into frozen VidLMs without compromising their existing capabilities. Due to limitations of the widely-used Video-Text Contrastive (VTC) loss for learning action knowledge, we introduce the DVDM objective to train the Knowledge Patcher. DVDM forces the model to encode the correlation between the action text and the correct ordering of video frames. Our extensive analyses show that Paxion and DVDM together effectively fill the gap in action knowledge understanding (~50% to 80%), while maintaining or improving performance on a wide spectrum of both object- and action-centric downstream tasks. The code and data will be made publicly available for research purposes at https://github.com/MikeWangWZHL/Paxion.git.

==> _backup/0_abstract_arxiv.tex <==
Action knowledge involves the understanding of textual, visual, and temporal aspects of actions. 
We introduce the \textbf{\ourbenchfull{} (\ourbench{})} containing two carefully designed probing tasks: Action Antonym and Video Reversal, which targets multimodal alignment capabilities and temporal understanding skills of the model, respectively. 
Despite recent video-language models' (\vidlm{}) impressive performance on various benchmark tasks,
our diagnostic tasks reveal their surprising deficiency (near-random performance) in \theKnowledge{}, suggesting that current models rely on object recognition abilities as a shortcut for action understanding.
To remedy this, we propose a novel framework, \textbf{\ours{}}, along with a new \textbf{\dvdm{} (\dvdmabbr{})} objective. 
The \ours{} framework utilizes a \textbf{\kp{}} network to encode new action knowledge and a \textbf{\kf{}} component to integrate the Patcher into frozen \vidlm{}s without compromising their existing capabilities.
Due to limitations of the widely-used Video-Text Contrastive (VTC) loss for learning \theKnowledge{}, we introduce the \dvdmabbr{} objective to train the \kp{}. \dvdmabbr{}
forces the model to encode the correlation between the action text and the correct ordering of video frames.
Our extensive analyses show that \ours{} 
and \dvdmabbr{} together effectively fill the gap in \theKnowledge{} understanding (\textasciitilde50\% $\rightarrow$ 80\%), while maintaining or improving performance on a wide spectrum of both object- and action-centric downstream tasks.\footnote{The code and data will be made publicly available for research purposes at \url{https://github.com/MikeWangWZHL/Paxion.git}}

==> _backup/2_physical_knowledge_benchmark_arxiv.tex <==
\section{\ourbenchfull{} (\ourbench{}): Do Video-Language Foundation Models Understand Action Knowledge?}
\label{sec:phy_benchmark}

%% combine the illustration with the backbone result figure

\input{figures/phy_bench_backbone_results}

To investigate the presence of action knowledge in state-of-the-art video-language foundation models, we propose the \textbf{\ourbenchfull{} (\ourbench{})}.
\ourbench{} comprises the \textbf{Action Antonym (AA)} and \textbf{Video Reversal (VR)} probing tasks, along with the \textbf{Object Replacement (OR)} baseline task. The probing tasks evaluate the \textit{multimodal and temporal correlations between an action text and a video}. The baseline task controls for the potential impact of domain mismatch.

We construct this benchmark by leveraging two existing open-domain video-language datasets, Ego4D~\cite{grauman2022ego4d} and Something-Something v2 (SSv2)~\cite{ssv2}, which provide fine-grained action annotations for each video clip.
Compared to a previous verb understanding probing benchmark~\cite{park2022exposing} based on MSRVTT~\cite{xu2016msrvtt} and LSMDC~\cite{LSMDC}, \ourbench{} is more action-oriented, larger in scale, and contains both ego-centric and third-person videos. Detailed statistics can be found in Appendix~\ref{App:benchmark_detail}. An illustration of each \ourbench{} task can be found in Figure~\ref{fig:benchmark_main}.

\vspace{-6pt}
\paragraph{Probing Task: Action Antonym (AA).}
\label{para:probing_task_AA}
The \textcolor{AA_txt_color}{Action Antonym} task probes the multimodal alignment of the action text and the video representation.
We formulate AA as a binary classification task that involves distinguishing the original text annotation from its altered version with the action replaced by its antonym, given the corresponding video clip.
For example, if the original text is \texttt{``Book \textcolor{pos}{falling} like a rock''}, the action antonym text would be \texttt{``Book \textcolor{neg}{rising} like a rock''}. 
We leverage the WordNet~\cite{miller1998wordnet} database and manually constructed mappings to automatically construct the antonym texts (details in Appendix~\ref{App:benchmark_detail}).

\vspace{-6pt}
\paragraph{Probing Task: Video Reversal (VR).}
\label{para:probing_task_VR}

The \textcolor{VR_txt_color}{Video Reversal} task probes the temporal understanding of actions. We formulate VR as a binary classification task, where given a video-text pair with at least one action and a reversed version of the video, the goal is to distinguish the original video from the reversed one. Achieving non-trivial performance on the Video Reversal task requires the model to understand the temporal sequence implied by the action.
%
The Video Reversal task also evaluates VLMs' abilities to identify violations of physical knowledge, as some clips defy expectation when reversed (e.g. a falling book becomes one which rises without any discernible cause).

\vspace{-6pt}
\paragraph{Baseline Task: Object Replacement (OR).}
\label{para:ref_task_OS}
\textcolor{OS_txt_color}{Object Replacement} is a binary classification task that requires the model to distinguish between the original text annotation and an altered version with objects tokens randomly replaced by other object tokens in the dataset. 
%
The Object Replacement task allows us to understand: (1) whether current \vidlm{}s rely on object recognition as a ``shortcut'' for video-text matching (i.e., if they have an object-biased representation), and 
(2) whether poor performance on Action Antonym can be attributed to domain mismatch (i.e., not being trained on Ego4D or SSv2) instead of a lack of \theKnowledge{}.

\subsection{Evaluating Video-Language Models on \ourbench{}}
We evaluate three recent video-language foundation models, \textbf{InternVideo}~\cite{internvideo}, \textbf{CLIP-ViP}~\cite{clipvip} and \textbf{Singularity-temporal}~\cite{singularity}\footnote{For simplicity, we use ``Singularity'' to represent ``Singularity-temporal'' in our figures and tables.}, on \ourbench{}. 
% brief description of models
InternVideo and CLIP-ViP have demonstrated state-of-the-art performance on various video-language tasks across 40+ datasets. Singularity-temporal is the multi-frame variant of Singularity~\cite{singularity}, equipped with an additional temporal encoder, which exhibits strong performance on tasks requiring find-grained temporal modeling. 

Despite their impressive improvements on video-language benchmarks, these models struggle to achieve non-trivial performance on Action Antonym and Video Reversal, as depicted in Figure~\ref{fig:benchmark_main}. The fact that they achieve significantly better performance on the Object Replacement task indicates a strong bias towards objects over actions, and affirms that the poor performance on AA is not solely a result of domain mismatch. The near-random performance on the VR task indicates a lack of basic temporal reasoning and physical knowledge.


These observations align with previous approaches~\cite{svo-probing, park2022exposing, Yuksekgonul2022WhenAW, verb-in-action} which show similar limitations in image-language models~\cite{clip,li2022blip} and earlier video-language models~\cite{MMT,luo2022clip4clip}. We find that high performance on video-language benchmarks does not necessarily equate to a stronger understanding of \theKnowledge{}.

==> _backup/4_knowledge_fuser_arxiv.tex <==
\section{Leveraging Patched \theKnowledgeCap{} for Downstream Tasks}
\label{sec:fuse}

In \S~\ref{sec:patch}, we showed that the \kp{} (\kpabbr{}) and \dvdmabbr{} objectives together effectively learn \theKnowledge{}-specific representations.
However, these representations are highly specialized to action understanding, which may not be optimal for general downstream tasks that require both object and action understanding. Thus, the remaining challenge is to \textit{retain the general VL capabilities of the backbone while leveraging the newly learned \theKnowledge{}.}

%
% the fuser figure
\input{figures/knowledge_fuser_alone}
%
One naive idea is to simply use the backbone embeddings whenever the task is less action-centric. However, it is difficult to decide when to use the backbone without prior knowledge of a given task. 
Further, using the backbone embeddings alone gives up the patched action knowledge that can be essential for certain downstream tasks, such as action recognition. 
%
In this section, we demonstrate that we can get the best of both worlds by fusing the action-centric representation from the \kp{} with the object-centric representation from the frozen backbone.

%
For this we introduce the second component of \ours{}, the \textbf{\kf{} (\kfabbr{})}, illustrated in \colorbox{KF_bg_color}{Figure~\ref{fig:knowledge_fuser_alone}}.  
The KF takes the pooled visual feature ($\boldsymbol{\mathcal{v}^*}$)
from the frozen VL backbone as the input query, and performs cross-attention with the extracted visual tokens ($\boldsymbol{\mathcal{V}}$) from the \kp{}.


\subsection{Experimental Setup}
\label{subsec:fuse_exp_setup}

% Video-text retrieval tasks are widely used to evaluate a model's general video-language alignment ability. However, as pointed out by several recent work~\cite{singularity, Yuksekgonul2022WhenAW}, traditional vision-language retrieval tasks suffer from ``static appearance bias'' and ``bag-of-words bias'' where using only a single frame from a video or shuffled text and patches can still achieve non-trivial or even state-of-the-art performance.

% To evaluate the true ability of understanding action dynamics and temporal modeling, we further include Video-to-Action Retrieval and Causal-Temporal VQA.

To evaluate the model's ability to retain general visual-linguistic capabilities while leveraging newly learned \theKnowledge{}, we consider a spectrum of video-language tasks with different emphases on object and action understanding. 
Specifically, we consider \textbf{Video-Text Retrieval} (SSv2-label~\cite{singularity}), which is object-centric and biased towards static appearances~\cite{Yuksekgonul2022WhenAW,singularity};
\textbf{Causal-Temporal VQA} (NExT-QA~\cite{nextqa}), which requires joint understanding of static objects and dynamic events; and \textbf{Video-to-Action Retrieval} (SSv2-template~\cite{singularity}, Temporal-SSv2~\cite{Temporal_dataset}), which is highly action-centric and temporal-intensive. A task is considered to be temporal-intensive if it cannot be solved without correct temporal information~\cite{Temporal_dataset}, e.g., reversed or shuffled frames. 
For example, as illustrated in Figure~\ref{fig:qualitative_examples}, the Video-to-Action Retrieval task obscures object names in the text, making it impossible to align text with a video based solely on objects. Moreover, it is impossible to distinguish ``approaching'' and ``moving away'' without considering the temporal ordering of the frames.

For \textbf{\ours{}}, we finetune the \kf{} jointly with the \kp{} on downstream tasks using VTC loss. By default, the \kpabbr{} in \ours{} is trained with VTC and DVDM losses (\S~\ref{subsec:dynamic_modeling_objective}). 
We include the baselines \textbf{KP-Transformer FT \scriptsize{[VTC]}} and \textbf{KP-Perceiver FT \scriptsize{[VTC]}}, which are both obtained by continuing to finetune the VTC-only \kpabbr{}s from Table~\ref{tab:probing_task_main_results} on downstream tasks. 
% for the same amount of epochs. 
Additionally, we compare \ours{} with \textbf{Side-Tuning}~\cite{side_tuning}, a Parameter-Efficient Finetuning (PEFT) method that could serve as an alternative to the \kfabbr{}. For the Side-Tuning variant, we initialize the "side-model" using the same \kp{} as in \ours{} and do alpha blending with the frozen backbone. Implementation and configuration details for each method and task can be found in Appendix~\ref{App:implementation_details}.
The results are shown in Tables~\ref{tab:downstream_task_retrieval} and \ref{tab:downstream_task_nextqa}.

%%% downstrea task results
\input{tables/downstream_task_retrieval}
\input{tables/downstream_task_nextqa}
%%%

\subsection{Analysis}
\label{subsec:fuse_quantitive_analysis}

\paragraph{\ours{} improves joint understanding of objects and actions.} Tables~\ref{tab:downstream_task_retrieval} and \ref{tab:downstream_task_nextqa} show that \ours{} outperforms both the \textit{Backbone} and the \textit{VTC-only baselines (KP-*)}. This indicates that \ours{} not only retains the original VL capabilities of the backbone, but also fills in the gap of the missing \theKnowledge{} by fusing the original representations with the patched ones. 
We corroborate this finding by observing more significant improvements on action-centric and temporal-intensive tasks, such as Temporal-SSv2 (+20\% @R1), compared to object-centric tasks, such as SSv2-label (+11\% @R1)\footnote{The scores are calculated between \ours{} and KP-Perceiver FT \scriptsize{[VTC]}. \footnotesize{The improvement @R1 for SSv2-label is averaged across $R1_{v2t}$ and $R1_{t2v}$}.}. \ours{} also outperforms Side-Tuning, highlighting the effectiveness of cross-attention for deep fusion. Specifically, the \kf{} allows us to attend to all extracted visual tokens from the \kp{} instead of only blending with pooled representations as in Side-Tuning.




% \subsection{Qualitative Analysis}
\vspace{-6pt}
\paragraph{Qualitative analysis.}
\input{figures/qualitative_examples_downstream_task}
Figure~\ref{fig:qualitative_examples} shows two qualitative examples on Temporal-SSv2 and NExT-QA. For the Temporal-SSv2 example, we find that the finetuned \kp{} trained with only VTC fails to distinguish \textit{``Moving away''} from \textit{``Approaching,''} while \ours{} trained with \dvdmabbr{} successfully correlates the seemingly expanding object with the action \textit{``Approaching''}. 
%
For the NExT-QA example, the question asks the model to identify what happens after the action \textit{``approached near the camera''}. The VTC baseline incorrectly selects the action \textit{``turn back to the toy,''} 
which happens before approaching the camera.  On the other hand, \ours{} successfully chooses \textit{``raised his hand to take the camera''}. This indicates a stronger understanding of both action dynamics in words such as \textit{``approach''} and the temporal ordering implied by words such as \textit{``after''}. Additional qualitative examples and analysis of failure cases can be found in Appendix~\ref{App:additional_qualitative_analysis}.

%% further analysis studies
\input{figures/vertical_bar_chart_analysis}
%%
\vspace{-6pt}
\paragraph{Disentangling the impact of Knowledge Patching and Fusing.} 
% To get an in-depth understanding of the synergy of Knowledge Patching and Fusing, 
We further investigate the disentangled impact of the \kf{} (\kfabbr{}) and the \kp{} (\kpabbr{}) with two ablation settings: (1) \textbf{KP+Finetune}, where instead of adding the \kfabbr{}, we directly \textit{finetune} the \kpabbr{} \textit{trained with \dvdmabbr{}} on downstream tasks; (2) \textbf{KP[VTC]+KF}, where we train the \kpabbr{} \textit{without \dvdmabbr{}} and then \textit{add the \kfabbr{}} upon it. 
% We compare the original \ours{} with these two ablated setting to answer the following questions: (1) What's the impact of the \kf{}. (2) What's the impact of the DVDM training. 
%
The results are shown in Figure~\ref{fig:further_analysis}, where the $\Delta$ score represents the relative difference of downstream task performance between our original \textbf{\ours{}} (Row 5 in Tables~\ref{tab:downstream_task_retrieval} and \ref{tab:downstream_task_nextqa}) and the two ablated settings. The key observations are as follows:
%
(1) \textbf{The \kf{} contributes more to object understanding.} From Figure~\ref{fig:further_analysis} Left, we find that the \kfabbr{} helps most when the tasks are more object-centric, e.g., SSv2-label. On highly action-centric tasks, e.g., Temporal-SSv2, directly using the action-knowledge-patched representation is preferable to fusing with the backbone representation.
%
(2) \textbf{Patching with action knowledge contributes more to action-centric understanding.} From Figure~\ref{fig:further_analysis} Right, we find that patching with action knowledge, i.e., training with \dvdmabbr{} objectives, contributes to better performance on downstream tasks that are more action-centric. 
Importantly, this result also indicates that the improvements observed in Tables~\ref{tab:downstream_task_retrieval} and \ref{tab:downstream_task_nextqa} do not come solely from adding the \kfabbr{}. However, if the task is more object-centric, such as SSv2-label, VTC training alone is sufficient.

%% summarize the following section
\vspace{-6pt}
\paragraph{Robustness to domain shift.} 
Learned \theKnowledge{} should be generalizable to unseen tasks and domains. However, this goal is difficult to realize with only domain-specific datasets like SSv2\cite{ssv2} which contains only 174 actions. Therefore, in Appendix~\ref{sec:cata_forget} we conduct experiments on zero-shot cross-domain transfer which demonstrate that the \kf{} in \ours{} increases robustness to domain shift and can introduce positive transfer during zero-shot inference.

==> _backup/7_conclusion_and_future_work_arxiv.tex <==
\section{Conclusions}
\label{sec:conclusion}
%conclusion
In this work we propose the \ourbench{} benchmark for evaluating models' understanding of \theKnowledge{}, and reveal a major deficiency in state-of-the-art video-language foundation models in this area. We then propose \ours{} to patch in such action knowledge without compromising models' existing capabilities. We show that \ours{} significantly improves the model's action understanding while achieving competitive or superior performance on downstream tasks. 

\section*{Limitations and Future Work}
One limitation of this work is that we only experimented with patching one type of knowledge. We intend to address this in future work, where we plan to expand \ours{} to patch broader aspects of physical knowledge such as object affordances and mental simulation, and to explore fusion with multiple learned Knowledge Patchers. Furthermore, we are interested in investigating the integration of interactive training into vision-language foundational models. This aims to overcome the inherent limitations posed by reliance on static data for training. Such an approach would equip these models with the ability to learn from and reason about visual and linguistic inputs in a more dynamic, interactive manner. Ultimately, this could significantly enhance their performance across a multitude of real-world tasks.

% \subsection{Conclusion}
% In this paper, we propose \ourbench{}, a benchmark that evaluates state-of-the-art video-language foundation models on their understanding of \theKnowledge{}. Our results indicate that current SOTA VLMs have limited understanding in these areas. To address this issue, we introduced Patch\&Fuse, a general knowledge patching framework that can learn specialized representations and fuse them with the backbone to improve downstream task performance.

% We also conducted an analysis of the model's robustness to catastrophic forgetting and found that the Fuse mechanism significantly reduces this issue. In fact, we achieved positive zero-shot cross-domain transfer by ensembling with the frozen backbone during inference.

% \subsection{Future Work}
% In future work, we plan to expand our benchmark to include other aspects of physical and world knowledge. This will help us better understand the strengths and limitations of current VLMs in modeling the real world.

% Additionally, we aim to introduce explicit interactive training for vision-language foundation models. This will enable the models to learn and reason about visual and linguistic inputs in a more interactive and dynamic way, which could potentially improve their performance on a range of tasks.

% \section{Limitations}
% limitation
% Currently, we only experimented with patching and fusing one type of knowledge. And the patched representation still struggles to bring positive transfer to a different domain as shown in \S~\ref{sec:cata_forget}. This indicates that the learned knowledge is entangled with domain-specific features.
% future work
% In future work, we plan to expand the \ours{} to patch broader aspects of physical knowledge such as object affordances and mental simulation, and explore fusing with multiple learned Knowledge Patchers.
% Additionally, we aim to investigate how to further disentangle knowledge learning with domain-specific features so that the learned knowledge is more generalizable to unseen tasks and domains.
% Additionally, we aim to explore more on dynamic pre-training objectives that  mimic the physical interactions for vision-language foundation models.

==> figures/patch_and_fuse_framework_illustration.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{image/patch_and_fuse_framework.pdf}
  \caption{Illustration of \ours{} framework, consisting of a \colorbox{KP_bg_color}{Knowledge Patcher} and a \colorbox{KF_bg_color}{Knowledge Fuser}. 
  % \colorbox{loss_bg_color}{\scriptsize{VTC}}, \colorbox{loss_bg_color}{\scriptsize{IDM}} and \colorbox{loss_bg_color}{\scriptsize{FDM}} indicate training objectives detailed in \S~\ref{sec:patch}.}
  \textit{\vtcabbr}, \textit{\idmabbr} and \textit{\fdmabbr} indicate \colorbox{train_obj_bg_color}{training objectives} detailed in \S~\ref{sec:patch}.
  }
  \label{fig:patch_and_fuse_framework}
\end{figure}

==> figures/radar_chart_dynamic_modeling_ablation_with_fuser.tex <==
% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\textwidth]{image/radar_chart__w_wout_dynamic_modeling.png}
%   \label{fig:radar_chart_fuser_ablation}
%   \caption{}
% \end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.445\textwidth}
        \includegraphics[width=\textwidth]{image/radar_chart__probing_task.png}
        \caption{radar chart for on Probing tasks (as a reminder for the reader that the IDM/FDM's main motivation is to learn the \theKnowledge{}-focused representation) \zhenhailong{Instead of showing this figure, maybe show the knowledge-fusers result on the probing tasks in the figure on the right}}
        \label{fig:radar_chart__probing_task}
    \end{subfigure}
    \hfill
    % \begin{subfigure}[t]{0.49\textwidth}
    %     \includegraphics[width=\textwidth]{image/radar_chart__w_wout_dynamic_modeling.png}
    %     \caption{\zhenhailong{TODO: caption}Adding knowledge fuser on VTC only knowledge patcher. Video Dynamic Modeling objectives introduces more benefits on more action-heavy and temporal-heavy tasks (SSv2-template, Temporal-SSv2)}
    %     \label{fig:radar_chart_fuser_ablation}
    % \end{subfigure}
    \begin{subfigure}[t]{0.49\textwidth}
        \includegraphics[width=\textwidth]{image/radar_chart__w_wout_dynamic_modeling_downstream_and_probing_task.png}
        \caption{Adding knowledge fuser on VTC only knowledge patcher. Video Dynamic Modeling objectives introduces more benefits on more action-heavy and temporal-heavy tasks (SSv2-template, Temporal-SSv2)}
        \label{fig:radar_chart_fuser_ablation}
    \end{subfigure}
    \caption{Impact of the Video Dynamic Modeling Objectives}
    \label{fig:bothfigures}
\end{figure}

==> figures/radar_chart_fuser_ablation.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{image/radar_chart__w_wout_knowledge_fuser.png}
  \label{fig:radar_chart_fuser_ablation}
  \caption{Impact of the Knowledge Fuser. knowledge fuser introduces more improvements on tasks that also require object understanding (SSv2-label, NExT-QA) which is complementary to the action-centric representation from the post-pretraining with video dynamic modeling\zhenhailong{TODO caption}}
\end{figure}

% \begin{wrapfigure}{r}{0.35\textwidth}
%   \centering
%   \includegraphics[width=0.35\textwidth]{image/radar_chart.png}
%   \caption{knowledge fuser introduces more improvements on tasks that also require object understanding (SSv2-label, NExT-QA) which is complementary to the action-centric representation from the post-pretraining with video dynamic modeling \zhenhailong{TODO: add color coding to the different tasks }}
%   \label{fig:radar_chart_fuser_ablation}
% \end{wrapfigure}
